Flamingo: Multi-Round Single-Server Secure Aggregation with Applications to Private Federated Learning

This paper introduces Flamingo, a system for secure aggregation of data across a large set of clients. In secure aggregation, a server sums up the private inputs of clients and obtains the result without learning anything about the individual inputs beyond what is implied by the final sum. Flamingo focuses on the multi-round setting found in federated learning in which many consecutive summations (averages) of model weights are performed to derive a good model. Previous protocols, such as Bell et al. (CCS '20), have been designed for a single round and are adapted to the federated learning setting by repeating the protocol multiple times. Flamingo eliminates the need for the per-round setup of previous protocols, and has a new lightweight dropout resilience protocol to ensure that if clients leave in the middle of a sum the server can still obtain a meaningful result. Furthermore, Flamingo introduces a new way to locally choose the so-called client neighborhood introduced by Bell et al. These techniques help Flamingo reduce the number of interactions between clients and the server, resulting in a significant reduction in the end-to-end runtime for a full training session over prior work. We implement and evaluate Flamingo and show that it can securely train a neural network on the (Extended) MNIST and CIFAR-100 datasets, and the model converges without a loss in accuracy, compared to a non-private federated learning system.

==> GNUmakefile <==
MAIN = main.tex

BASE := $(basename $(MAIN))
SRCEXT := $(patsubst $(BASE).%,%,$(MAIN))
BIBFILES := $(wildcard bib/*.bib)
STYLINK := $(notdir $(wildcard *.sty))
STYFILES := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES))
PLOT_SCRIPTS := $(wildcard scripts/*) $(wildcard scripts/proc_rslt/*)
PLOT_LOGS := $(wildcard logs/*.log)
PLOTS := $(patsubst logs/%.log, graphs/%.pdf, $(PLOT_LOGS))

LATEX = pdflatex
BIBTEX = bibtex -min-crossrefs=1000
PS2PDF = ps2pdf


# by default, not extended mode
# change this to 1 if you want extended mode by default
EXTENDED ?= 0
ifeq ($(EXTENDED),1)
EXTDEF := \def\buildextended{}
else
EXTDEF := 
endif

# by default, editing marks
# change this to 0 if you want no edit marks by default
EDITING ?= 1
ifeq ($(EDITING),1)
EDITDEF := 
else
EDITDEF := \def\noeditingmarks{}
endif

# put latexmk in auto mode?
AUTO ?= 0
ifeq ($(AUTO),1)
AUTODEF := -pvc
else
AUTODEF :=
endif

all: $(BASE).pdf

#.headline:
#	$(MAKE) -C headline

#.images: headline/headline.eps  $(addsuffix /*.eps,$(IMAGES)) $(addsuffix /*.tex,$(IMAGES))
#	for i in $(IMAGES); do $(MAKE) -C $$i; done
#	touch $@

graphs/%.pdf: scripts/%.rb logs/%.log
	mkdir -p graphs
	$< | gnuplot > $@.eps
	epstopdf --outfile=$@ $@.eps
	rm $@.eps

.SECONDEXPANSION:
$(FIGURES): %.tex: scripts/%.sh scripts/proc_rslt/%.rb $$(wildcard %-skeleton.tex) $$(wildcard logs/%/*.txt)
	mkdir -p graphs
	$< $(lastword $+)
	touch $@

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

$(BASE).pdf: %.pdf: %.$(SRCEXT) $(TEXFILES) $(BIBFILES) $(FIGURES) $(PLOT_SCRIPTS) $(PLOTS)
	echo '$(EXTDEF)$(EDITDEF)\input{$<}' > $(BASE).tltx
	latexmk $(AUTODEF) -pdf -pdflatex='pdflatex --enable-write18 %O %S' $(BASE).tltx
	rm -f $(BASE).tltx

show: $(BASE).pdf
	xpdf -fullscreen $(BASE).pdf

osx: $(BASE).pdf
	open $(BASE).pdf

double:
	for i in $(TEXFILES); do perl double.pl $$i; done	

clean:
		rm -f graphs/* scripts/dat/*
		rm -f $(BASE).ps $(BASE).pdf
		rm -f *.dvi *.aux *.log *.bbl *.blg *.lof *.lot *.toc *.bak *.out .images $(BASE).fdb_latexmk $(BASE).fls $(BASE).tltx
		for i in $(IMAGES); do $(MAKE) -C $$i clean; done

spell:
	make clean
	for i in $(wildcard *.tex); do aspell -p ./aspell.words -c $$i; done


==> figures/F-semi.tex <==

\begin{figure}
 \begin{tcolorbox}[enhanced, boxsep=1mm, left= 0mm, right=0.5mm, title={\textbf{\footnotesize Functionality $\Fsemi$}}]
    \linespread{1.4}
    \footnotesize
    
    Parties: clients $1, \ldots, N$ and a server.
    
    Parameters: corrupted rate $\eta$, dropout rate $\gamma$. 
    
    \begin{myitemize2}
    
    

        \item $\Fsemi$ receives from the adversary $\Adv$ a set of corrupted parties,
                denoted as $\mathcal{C} \subset[N]$, where $|\mathcal{C}|/N \le \eta$.
        \item For each round $t\in [T]$:
            \begin{enumerate}
                \item  $\Fsemi$ receives a random subset $S_t\subset [N]$, a set of dropout clients $\mathcal{O}_t \subset S_t$, 
                where $|\mathcal{O}_t|/|S_t| \le \delta$ and $|\mathcal{C}|/|S_t| \le \eta$,
                and inputs $\vec{x}_{i,t}$ for client $i \in S_t \backslash \mathcal{O}_t$.
                
                \item  $\Fsemi$ outputs $z_t = \sum_{i \in S_t\backslash (\mathcal{O}_t \cup \mathcal{C})} \vec{x}_{i, t}$. 
            
            \end{enumerate}
           
        
    \end{myitemize2}
    
    \end{tcolorbox}
\caption{Ideal functionality for Flamingo, semi-honest version.}
\label{fig:F-ideal-semi}
\end{figure}


==> figures/Frand.tex <==

\begin{figure}
 \begin{tcolorbox}[enhanced, boxsep=1mm, left= 0mm, right=0.5mm, title={\textbf{\footnotesize Functionality $\Frand$}}]
    \linespread{1.4}
    \footnotesize
    \begin{myitemize2}
        \item $\Frand$ samples a random value $v$ in $\{0,1\}^\kappa$.
        \item $\Frand$ sends $v$ to the adversary.
        
         If the adversary replies \texttt{continue}, $\Frand$ sends $v$ to honest parties;
         if the adversary replies \texttt{abort}, $\Frand$ sends \texttt{abort} to honest parties.
    \end{myitemize2}
    
    \end{tcolorbox}
\caption{Ideal functionality for generating global randomness.}
\label{fig:Frand}
\end{figure}

==> figures/Fsumt.tex <==

\begin{figure}
 \begin{tcolorbox}[enhanced, boxsep=1mm, left= 0mm, right=0.5mm, title={\textbf{\footnotesize Functionality $\mathcal{F}_{\text{sum-robust}}^{(t)}$}}]
    \linespread{1.4}
    \footnotesize
    
    Parties: clients in $S_t$ and a server.
    
    Parameters: dropout rate $\delta$ and malicious rate $\eta$ over $|S_t|$ clients.
    
    \begin{myitemize2} 

        \item $\mathcal{F}_{\text{sum-robust}}^{(t)}$ receives a set $\mathcal{O}_t$ 
        such that $|\mathcal{O}_t| / |S_t| \le \delta$,
        and a set of corrupted parties, $\mathcal{C}$;
        and $\vec{x}_{i, t}$ from client $i\in  S_t \backslash (\mathcal{C} \cup \mathcal{O}_t) $.
        
        Depending on whether the server is corrupted by the adversary $\Adv$ or not, there are two cases:
        \begin{enumerate}
                    \item If the server is not corrupted by $\Adv$, 
                    then $\Fmal$ outputs $z_t = \sum_{ i \in S_t \backslash (\mathcal{C} \cup \mathcal{O}_t)} \vec{x}_{i, t}$;
                    \item If the server is corrupted by $\Adv$, then $\Fmal$ asks $\Adv$ for a set: 
                if $\Adv$ replies with a set $M_t \subseteq S_t$ such that $|M_t|/|S_t| \ge 1-\delta$, then $\Fmal$ outputs
                $z_t' = \sum_{i\in M_t \backslash \mathcal{C}} \vec{x}_{i,t} $; otherwise sends \texttt{abort} to all honest clients.
        
        \end{enumerate}
    \end{myitemize2}
    
    \end{tcolorbox}
\caption{Ideal functionality for a single round $t$ in the collection phase with robustness.}
\label{fig:Fsumt}
\end{figure}
